Global results for linear waves on expanding Kerr and Schwarzschild de Sitter cosmologies

In this global study of solutions to the linear wave equation on Schwarzschild de Sitter spacetimes we attend to the cosmological region of spacetime which is bounded in the past by cosmological horizons and to the future by a spacelike hypersurface at infinity. We prove an energy estimate capturing the expansion of that region which combined with earlier results for the static region yields a global boundedness result for linear waves. It asserts that a general finite energy solution to the global initial value problem has a limit on the future boundary at infinity that can be viewed as a function on the standard cylinder with finite energy, and that moreover any decay along the cosmological horizon is inherited along the future boundary. In particular, we exhibit an explicit nonvanishing quantity on the future boundary of the spacetime consistent with our expectations for the nonlinear stability problem. Our results apply to a large class of expanding cosmologies near the Schwarzschild de Sitter geometry, in particular subextremal Kerr de Sitter spacetimes.

==> intro.tex <==
The primary impetus for the study of the linear wave equation on black hole spacetimes is that some aspects of the stability or instability of dynamical black holes are already foreshadowed in the global behaviour of linear waves \cite{dr:bhslp,a:in}.
While the resolution of the \emph{black hole stability conjecture} has remained elusive for many years \cite{d:bhsp}, the motivation for the linear theory developed in this paper is largely drawn from our expectation that the nonlinear stability problem is within reach in the context of \emph{expanding spacetimes}.

The favorable effect of a \emph{positive} cosmological constant was first recognized by Friedrich in his proof of the stability of the de Sitter solution \cite{f:ds}. Since then the conformal method has been extended to scalar field models \cite{hr:s,k:fs}, and the stabilizing effect of the cosmological constant on perfect fluids has been established in \cite{rs:siee,s:se}, (and \cite{kl:pureradiation} in the pure radiation case). However, the original approach of \cite{f:ds} to the study of solutions to the Einstein equations close to de Sitter is limited to the class of \emph{compact} initial data, and does not have implications for initial data globally close to the \emph{Schwarzschild}-de Sitter solution, which presents us with an entirely different global geometry.

It is for this reason that in this paper we insist on a \emph{global} perspective on the study of the linear wave equation on Schwarzschild de Sitter black hole spacetimes. We may think of this spacetime as an infinite chain of black hole interiors, \emph{static} black hole exterior regions, and \emph{expanding} or \emph{cosmological} regions separated by event horizons and cosmological horizons respectively \cite{gh:ceh}. While the static region has already been studied intensively \cite{bh:sds,dr:sds,mbv:sds} (and the black hole interior is only of secondary interest to the stability problem, see e.g.~\cite{dr:c}), we focus in this paper on what shall be referred to as ``the expanding region'' bounded in the past by cosmological horizons and to the future by a \emph{spacelike} hypersurface (see figure \ref{fig:cauchyexpanding}).

\begin{figure}
\includegraphics{cauchy_expanding}
\caption{Global geometry of Schwarzschild de Sitter. The expanding region is the domain bounded in the past by the cosmological horizons $\mathcal{C}^+$ and $\bar{\mathcal{C}^+}$ and to the future by the spacelike hypersurface $\Sigma^+$. $\mathcal{H}^+$ and $\bar{\mathcal{H}}^+$ denote the event horizons of the adjacent black hole interiors.}
\label{fig:cauchyexpanding}
\end{figure}

The expanding region of Schwarzschild de Sitter is foliated by spacelike hypersurfaces of constant area radius. We exhibit in this paper an energy of linear waves which is \emph{monotone} with respect to this foliation. Moreover, we show that any solution to the linear wave equation with initially finite energy on a Cauchy hypersurface $\Sigma$ lying in the past of the future boundary $\Sigma^+$ of the expanding region (such that $\Sigma^+$ is in the domain of dependence of $\Sigma$, see figure \ref{fig:cauchyexpanding}) \emph{attains a limit on $\Sigma^+$ viewed as a function on the standard cylinder $\mathbb{R}\times\mathbb{S}^2$}. In addition, it will be shown that as a consequence of the presence of a ``global redshift effect'' any decay along the cosmological horizon will be inherited along the future boundary of the spacetime. The ideas of the proof originate in my treatment of linear waves on de Sitter spacetimes \cite{vs:thesis} which is summarized in the epilogue of this paper.


==> sitter.tex <==
The global study of linear waves on cosmological black hole spacetimes initiated in this paper applies to Schwarzschild de Sitter spacetimes with positive mass $m$ in the range $0<3m\sqrt{\Lambda}<1$. In this epilogue I present analogous results for solutions to the Klein-Gordon equation
\begin{equation}
  \label{eq:ds:kg}
  \Box_g\psi=\m\psi\,,\qquad\m\geq 0\,,
\end{equation}
in the case where the background spacetime has vanishing mass $m=0$, i.e.~on de Sitter spacetimes $(\Ml,g)$ with positive cosmological constant $\Lambda> 0$.

It is well-known that the de Sitter cosmology is \emph{homogeneous}, or in other words as opposed to Schwarzschild de Sitter spacetimes not only spherically symmetric with respect to a distinguished centre (the centre of the black hole), but in fact spherically symmetric with respect to \emph{any} timelike geodesic. The manifold $\Ml$ can be embedded as a hyperboloid in $\mathbb{R}^5$ with spacially \emph{compact} sections diffeomorphic to $\mathbb{S}^3$, highlighting its interpretation as an expanding universe since its discovery in \cite{ds:astro}. Alternatively $\Ml$ appears as a canonical constant curvature spacetime and can be cast as a subset of Minkowski space endowed with a metric \emph{conformal} to the flat metric (see e.g.~\cite{ch:mpI}), which provides the point of departure for the conformal method. In particular, for a specific value of $\m$ the problem \eqref{eq:ds:kg} is conformally equivalent to the wave equation on Minkowski space (c.f.~Remark~\ref{remark:conformal}); see e.g.~in the work of \cite{b:strichartz,b:strichartz:a}.

However, with applications to the \emph{Schwarzschild-}de Sitter geometry in mind  we \emph{choose} not to make use of the homogeneity of the spacetime $(\Ml,g)$, by \emph{fixing} a centre of symmetry. (We adopt the point of view on de Sitter as the subfamily of the Schwarzschild de Sitter family $(\M,g)$ corresponding to a mass parameter $m=0$.) This has the advantage that a causal geometry emerges (with respect to a chosen observer) that shares some essential features with the Schwarzschild de Sitter geometry, in particular the existence of an expanding region in the sense described above, and allows us to exemplify our approach in a simpler setting. In the following I present an alternative construction of the global redshift vectorfield which may be useful in future applications, and I demonstrate that my results for the wave equation can easily be extended to the Klein-Gordon equation, irrespective of the specific value of $\m$.

\subsection{Global results for the wave equation on de Sitter spacetimes}
In adopting the point of view outlined above we are lead to the following description of the de Sitter cosmology with positive cosmological constant $\Lambda>0$ (as depicted in figure~\ref{figure:thm:ds}) \cite{gh:ceh}.

Let $\Gamma$ be a timelike geodesic in $(\Ml,g)$. We denote by $r$ the area radius of the round spheres defined by the orbits of the $\mathrm{SO}(3)$ subgroup of the isometry group that leaves $\Gamma$ invariant, and by $\Omega_{(i)}$ the generators of this group action.
Consider the level sets $\Sigma_r$ of the area radius function $r$ on $(\Ml,g)$.
These are timelike hypersurfaces for $r<\chin$, and null hypersurfaces for $r=\chin$. The domain $r<\chin$ is a static region of spacetime in the intersection of the timelike future and past of $\Gamma$, and as such endowed with a timelike Killing vectorfield $T$, which  is tangential to $\Sigma_r$.
We denote by $\mathcal{C}^+$ the future boundary of the past of $\Gamma$, and by $\mathcal{C}^-$ the past boundary of the future of $\Gamma$; these are the cosmological horizons of $\Gamma$.
The level sets $\Sigma_r$ are spacelike hypersurfaces for $r>\chin$. More precisely, the hypersurfaces $\Sigma_r$ are topologically cylinders that foliate the cosmological region $r>\chin$, and $T$ extends to a global Killing vectorfield tangential to $\Sigma_r$. We shall refer to the component of the cosmological region that lies in the future of the static domain as the expanding region.  In this domain the metric takes the form
\begin{equation}
  \label{eq:ds:intro:metric}
  g=-\phi^2\ud r^2+\gb{r}=-\frac{1}{\frac{\Lambda}{3}r^2-1}\ud r^2+\gb{r}\,,
\end{equation}
where $\gb{r}$ is the induced metric on $\Sigma_r$, a Riemannian metric conformal to the standard cylinder; in fact $\lim_{r\to\infty}\:r^{-2}\,\gb{r}=\stackrel{\circ}{g}$ is the standard metric on the cylinder $\mathbb{R}\times\mathbb{S}^2$.
We denote by $\Sigma^+$ the future timelike boundary of the expanding region endowed with the rescaled metric $\cg$.

\begin{figure}
\includegraphics{penrosedesitter}
\caption{Penrose diagram of de Sitter depicted as a spherically symmetric spacetime with respect to a chosen timelike geodesic $\Gamma$.}
\label{figure:thm:ds}
\end{figure}

\begin{thm}
\label{thm:ds:energy}  
Let $\Sigma$ be a spacelike hypersurface with normal $n$ in de Sitter $(\Ml,g)$, and $\Gamma$ a timelike geodesic with cosmological horizons $\mathcal{C}^+$ and $\mathcal{C}^-$, and assume that $\Sigma$ crosses the horizons to the future of $\mathcal{C}^+\cap\mathcal{C}^-$ (see figure \ref{figure:thm:ds}).
Let moreover $\psi$ be a solution to the linear wave equation \eqref{eq:ds:kg} for either $\m=0$ or $\m\geq 2\frac{\Lambda}{3}$ with initial data prescribed on $\Sigma$ such that
\begin{equation}
  \label{eq:thm:energy:condition}
  D[\psi]\doteq\int_{\Sigma}\biggl\{J^n[\psi]\cdot n+\m\psi^2\biggr\} <\infty\,.
\end{equation}
Then we have the global bound
\begin{equation}
  \label{eq:thm:geb:b}
  \int_{\Sigma^+}\biggl\{\sq{T\cdot\psi}+\sum_{i=1}^3\sq{\Oi{i}\psi}+\m\sq{r\psi}\biggr\}\dm{\cg}\leq C(\Lambda,\Sigma)\,D[\psi]
\end{equation}
on the future boundary $\Sigma^+$, where $C$ is a constant that only depends on $\Lambda$ and the initial hypersurface $\Sigma$.
\end{thm}

In the case $\m=0$ we have the existence of the limit of $\psi$ on $\Sigma^+$ in the norm defined by \eqref{eq:thm:geb:b} analogous to Thm.~\ref{thm:sds} by the density argument described in Section~\ref{sec:limit}. Since $r\to\infty$ along any curve that terminates on $\Sigma^+$ this limit is identically zero for $\m\geq 2\frac{\Lambda}{3}$. Note that $\m=\mc$ is precisely the conformal value of $\m$.

\emph{Identical conclusions to Corollary~\ref{thm:sds:pointwise} for pointwise bounds are drawn in the case $\m=0$ in view of the Sobolev embedding derived in Appendix~\ref{a:coercivity}, and the inherent decay result of Corollary~\ref{cor:decay} holds true in identical terms for the wave equation on the expanding region of de Sitter.}

\begin{rmk} \label{remark:conformal}
For the specific value $\m=2\frac{\Lambda}{3}$ the Klein-Gordon equation \eqref{eq:ds:kg} is conformal to the wave equation on Minkowski space $(\mathbb{R}^{3+1},\eta)$.
More precisely, recall that we can cast de Sitter as the subset
\begin{equation}
  \mathcal{M}=\Bigl\{x\in\mathbb{R}^{3+1}\,:\ \langle x,x\rangle=-(x^0)^2+(x^1)^2+(x^2)^2+(x^3)^2>-\frac{4}{\kappa}\Bigr\}\,,
\end{equation}
endowed with the metric $g=\Omega^2\,\langle\ud x,\ud x\rangle=\Omega^2\,\eta$ where
\begin{equation}
  \Omega=\frac{1}{1+\frac{\kappa}{4}\langle x,x\rangle}\,,\quad\text{and } \kappa=\frac{\Lambda}{3}\,.
\end{equation}
The following well-known fact demonstrates the significance of the conformal value, and allows us to read off qualitatively our main result in this special case. 

\emph{Let $\psi$ be a solution to $\Box_g\psi=2\kappa\,\psi=2\frac{\Lambda}{3}\,\psi$, then $\tilde{\psi}=\Omega\,\psi$ is a solution to $\Box_{\tilde{g}}\tilde{\psi}=0$ where $\tilde{g}=\Omega^{-2}g=\eta$ is the Minkowski metric.}

For a solution of the classical wave equation $\Box_\eta\tilde{\psi}=0$ will assume nonvanishing values on the boundary $\langle x,x\rangle=-4/\kappa$. The decay of $\psi$ is then entirely due to the conformal factor $\Omega$, i.e.~the ``expansion'' of the spacetime.
\end{rmk}


\subsection{Remarks on the proof of theorem.}

The central idea of the proof is the construction a \emph{global} redshift vectorfield that captures the \emph{expansion} of the spacetime in the region $r>\chin$. We establish that for any solution to \eqref{eq:ds:kg} with $\m\geq 0$,
\begin{multline}
  \label{eq:proof:ee:expanding}
  \int_{\Sigma_{r_2}}\phi\Biggl\{\phi^2\bigl(T\cdot\psi\bigr)^2+\lvert\nablab\psi\rvert^2+\m\psi^2\Biggr\}\dm{\gb{r_2}}\leq\\
    \leq\int_{\Sigma_{r_1}}\phi\Biggl\{\phi^2\bigl(T\cdot\psi\bigr)^2+\frac{1}{\phi^2}\bigl(\dd{r}{\psi}\bigr)^2+\lvert\nablab\psi\rvert^2+\m\psi^2\Biggr\}\dm{\gb{r_1}}
\end{multline}
for all $r_2>r_1>\chin$, where $\phi$ is the lapse function \eqref{eq:lapse} of the foliation $\Sigma_r$. The multiplier vectorfield that gives rise to this bound is here defined in a double null foliation which casts the global redshift effect as an extension of the local redshift effect, and provides an alternative proof of Prop.~\ref{prop:r:expanding}. This part of the proof, besides the general modification for the inclusion of the Klein-Gordon mass term shall be discussed in Sections~\ref{sec:ds:dn}-\ref{sec:ds:expanding:c}.

A secondary aspect is --- as in the corresponding Schwarzschild de Sitter problem --- the use of the \emph{local} redshift effect in the vicinity of the cosmological horizons $\mathcal{C}^+$, $\mathcal{C}^-$ in order to obtain control on the right hand side of \eqref{eq:proof:ee:expanding} (for $r_1-\chin>0$ chosen suitably small) in terms of an energy on $\mathcal{C}^+$. The analogous discussion to Section~\ref{sec:sds:localredshift} shall not be repeated here (the reader is referred to \cite{vs:thesis}), but we point out that this step crucially depends on the positivity of the surface gravity,
\begin{equation}
  \kappa_\mathcal{C}=\sqrt{\frac{\Lambda}{3}}>0\,,
\end{equation}
of the Killing horizons $\mathcal{C}^+$, and $\mathcal{C}^-$.

In order to close the estimate we require the analogous statement of Prop.~\ref{prop:r:static} for the static domain in the intersection of the timelike future and past of $\Gamma$. We have simplified the proof of \cite{dr:sds} to establish the proposition in the case $m=0$, independently of the work presented in this paper. 

\begin{prop}\label{prop:ds:static}
  Let $\Sigma_0$ be a spacelike hypersurface with normal $n$ in the static region of de Sitter crossing the cosmological horizon $\mathcal{C}^+$ to the future of the sphere $\mathcal{C}^+\cap\mathcal{C}^-$, and denote by $\mathcal{C}_0^+=J^+(\Sigma_0)\cap\mathcal{C}^+$ the segment of the cosmological horizon to the future of $\Sigma_0$. Then there exist a strictly timelike vectorfield $N$ (normalized in the sense that $g(T,N)$ is constant on $\mathcal{C}_0^+$) and a constant $C(\Lambda, \Sigma_0)$ such that for all solutions to the wave equation \eqref{eq:ds:kg} we have
  \begin{equation}
    \int_{\mathcal{C}^+_0}\Bigl\{{}^\ast J^N[\psi]+\m\psi^2\Bigr\} \leq C(\Lambda,\Sigma_0)\,\int_{\Sigma_0}\Bigl\{J^n[\psi]\cdot n+\m\psi^2\Bigr\}\,,
  \end{equation}
provided either $\m=0$ or $\m\geq\mc$.
\end{prop}

The complete proof of this fact can be found in my thesis \cite{vs:thesis}. It amounts to an \emph{integrated local energy estimate} that is proven using an adapted Morawetz vectorfield \cite{mora:p,dr:c}. The introduction of a virial current is compelled by the behaviour of the local redshift current which fails to remain positive away from the horizon. Conversely an integrated local energy estimate for the static region that holds up the horizon can only be proven in conjunction with a redshift estimate. For an explanation of the subtle interplay between the two currents, and the technical details involved see \cite{vs:thesis}. 

It is in this part of the proof that the condition $\m\geq\mc$ is introduced. The proof of Prop.~\ref{prop:ds:static} in the case $\m=0$ relies on a Poincar\'e inequality which for $\m>0$ is conveniently replaced by a lower bound on $\m$ \cite{vs:thesis}. We expect that this gap in the range of valid values for $\m$ is due to a shortcoming of the proof of Prop.~\ref{prop:ds:static} which can be amended by an alternative proof, and that it is not essential for the finial result as stated in Thm.~\ref{thm:ds:energy} \emph{in view of \eqref{eq:proof:ee:expanding} which holds true for the entire range of mass values $\m\geq 0$}.

With the global and local redshift estimates in place we can then proceed as discussed in Section~\ref{sec:r:integral}.
Since we have again formally \eqref{eq:sds:overview:volumeform}, and the coercivity equality on the sphere (see Appendix \ref{a:coercivity}),
$r^2\sqv{\nablab\psi}=\sum_{i=1}^3\sq{\Oi{i}\psi}$, 
we are allowed to take the limit in \eqref{eq:proof:ee:expanding} as $r_2$ tends to infinity, to conlude on the finiteness of the following quantity:
\begin{multline}
  \label{eq:proof:limit}
  \lim_{r\to\infty}\int_{\Sigma_r}\phi\Biggl\{\phi^2\bigl(T\cdot\psi\bigr)^2+\lvert\nablab\psi\rvert^2+\m\psi^2\Biggr\}\dm{\gb{r_2}}=\\
  =\int_{\Sigma^+}\biggl\{\frac{3}{\Lambda}\sq{T\cdot\psi}+\sum_{i=1}^3\sq{\Oi{i}\psi}+\m\sq{r\psi}\biggr\}\dm{\cg}\,.
\end{multline}

We shall conclude our remarks on Theorem~\ref{thm:ds:energy} with the proof of \eqref{eq:proof:ee:expanding} using a global double null coordinate system for $(\Ml,g)$.

\subsection{Double null foliation of de Sitter}
\label{sec:ds:dn}

The general discussion of spherically symmetric spacetimes with cosmological constant $\Lambda>0$ reveals that in the case
\begin{equation}
  \label{eq:m:zero}
  m=0\,,
\end{equation}
the manifold $\Ml$ can be covered by a single chart.
On one hand, we find immediately for \eqref{eq:sds:tortoise},
\begin{equation}
  \label{eq:tortoise}
  r^\ast=\int\frac{1}{1-\frac{\Lambda r^2}{3}}\ud r=\frac{1}{2}\ch\log\Bigl\vert\frac{1+\sqrt{\frac{\Lambda}{3}}r}{1-\sqrt{\frac{\Lambda}{3}}r}\Bigr\vert\,,
\end{equation}
and on the other hand, we may choose
\begin{equation}
  \label{eq:rsol}
  r^\ast=\frac{1}{2}\ch\log\frac{1}{\lvert u v\rvert}\,,
\end{equation}
so that we can express $r$ explicitly as a function of $u$, $v$ as follows:
\begin{equation}
  \label{eq:r}
  r=\ch\frac{1+uv}{1-uv}\,.
\end{equation}
Finally, using \eqref{eq:massfunction},
\begin{equation}
  \label{eq:omega}
  \Omega^2=\frac{3}{\Lambda}\Bigl(1+\sqrt{\frac{\Lambda}{3}}r\Bigr)^2\,,
\end{equation}
the de Sitter metric takes the form:
\begin{equation}
  \label{eq:desitter}
  g=-\frac{3}{\Lambda}\Bigl(1+\sqrt{\frac{\Lambda}{3}}r\Bigr)^2\ud u\,\ud v+r^2\g\,.
\end{equation}
For reference, we also note
\begin{equation}
  \label{eq:ds:dr}
  \frac{\partial r}{\partial u}=\ch\frac{2v}{(1-uv)^2}\qquad  \frac{\partial r}{\partial v}=\ch\frac{2u}{(1-uv)^2}\quad
\end{equation}
and
\begin{equation}
  \label{eq:ri}
  \frac{1}{1+\sqrt{\frac{\Lambda}{3}}r}=\frac{1-uv}{2}\,.
\end{equation}

The very purpose of the representation of $\Ml$ in this manner is the obvious analogy of the expanding region $\mathcal{R}^+\doteq\{(u,v):u>0,v>0,uv<1\}$ to the corresponding region in $(\M,g)$ for $m>0$ as discussed in Section~\ref{sec:sds:foliation}, which is similarly foliated by the level sets of the area radius
\begin{equation}
  \mathcal{R}^+=\bigcup_{r>\ch}\Sigma_{r}\,;\qquad\Sigma_{r}\doteq\Bigl\{(u,v):\ch\frac{1+uv}{1-uv}=r\Bigr\}\,.
\end{equation}
Here the gradient vectorfield \eqref{eq:sds:r:grad} of the time function $r$ is given by
\begin{equation}
  V=\frac{\Lambda}{3}\Bigl(u\pd{u}+v\pd{v}\Bigr)\,,
\end{equation}
and we obtain for the lapse function of the foliation $\Sigma_r$,
\begin{equation}
  \label{eq:lapse}
  \phi=\frac{1}{\sqrt{-g(V,V)}}=\frac{1}{\sqrt{\frac{\Lambda}{3}r^2-1}}\,,
\end{equation}
which yields \eqref{eq:ds:intro:metric} as desired.


\subsection{Energy estimates and global redshift effect in the expanding region}
\label{sec:ds:expanding}

We shall give here an exposition of the energy estimates for the expanding region in purely geometric terms, and complement those by calculations in the following section using the specific coordinates of Section~\ref{sec:ds:dn}.

$\boldsymbol{\m=0}$.
Consider the energy current $J^M$ associated to the multiplier
\begin{equation}
  \label{eq:M:hom}
  M=\bar{Y}+Y\,,
\end{equation}
where
\begin{equation}
  \label{eq:YY}
  \bar{Y}=\frac{1}{\dd{u}{r}}\pd{u}\,,\qquad Y=\frac{1}{\dd{v}{r}}\pd{v}\,.
\end{equation}
We can show that for any solution of \eqref{eq:ds:kg}, this is a positive current, i.e.
\begin{equation}
  \label{eq:M:hom:div}
  \nabla\cdot J^M\geq 0\,.
\end{equation}
Therefore, by the energy identity for $J^M$, 
\begin{equation}
  \label{eq:M:hom:energy}
  \int_{\Sigma_{r_2}}J^M\cdot n\,\dm{\gb{r_2}}\leq  \int_{\Sigma_{r_1}}J^M\cdot n\,\dm{\gb{r_1}}
\end{equation}
which yields our energy estimate for solutions to the wave equation.

\begin{prop}\label{prop:geb}
Let $\psi$ be a solution to the wave equation \eqref{eq:ds:kg}, $\m=0$, then
\begin{equation}
  \label{eq:prop:geb}
  \int_{\Sigma_{r_2}}\phi\biggl\{\phi^{2}\bigl(T\cdot\psi\bigr)^2+\lvert\nablab\psi\rvert^2\biggr\}\dm{\gb{r_2}}
  \leq\int_{\Sigma_{r_1}}J^M\cdot n\,\dm{\gb{r_1}}
\end{equation}
for any $r_2>r_1>\ch$.
\end{prop}

It is equivalent to consider the multiplier
\begin{equation}
  \label{eq:M:redshift}
  M=\frac{1}{1+\sqrt{\frac{\Lambda}{3}}r}\,\bigl(\bar{Y}+Y\bigr)\,.
\end{equation}
The associated energy current has the redshift property
\begin{equation}
  \label{eq:redshiftM}
  \phi\:\nabla\cdot J^M\geq\frac{\sqrt{\frac{\Lambda}{3}}}{1+\sqrt{\frac{\Lambda}{3}}r}J^M\cdot n
\end{equation}
for any solution of the wave equation; (here $n$ denotes the unit normal to $\Sigma_r$).
The energy identity for $J^M$ then implies, in view of the coarea formula,
\begin{multline}
  \int_{\Sigma_{r_2}}J^M\cdot n\,\dm{\gb{r_2}}+\int_{r_1}^{r_2}\ud r \frac{\sqrt{\frac{\Lambda}{3}}}{1+\sqrt{\frac{\Lambda}{3}}r}\int_{\Sigma_r}J^M\cdot n\,\dm{\gb{r}}\leq\\
  \leq\int_{\Sigma_{r_1}}J^M\cdot n\,\dm{\gb{r_1}}\,.
\end{multline}
By a Gronwall-type inequality  we obtain
\begin{equation}
\label{ineq:wenergy}
\bigl(1+\sqrt{\frac{\Lambda}{3}}r_2\bigr)\int_{\Sigma_{r_2}}J^M\cdot n\,\dm{\gb{r_2}}\leq\bigl(1+\sqrt{\frac{\Lambda}{3}}r_1\bigr)\int_{\Sigma_{r_1}}J^M\cdot n\,\dm{\gb{r_1}}\,,
\end{equation}
which precisely reproduces \eqref{eq:prop:geb}.
In fact, as we shall see below, the argument applies to any multiplier
\begin{equation}
  \label{eq:Malpha}
  M=\lr^\alpha\,\bigl(\bar{Y}+Y\bigr)\qquad(\alpha<0)\,;
\end{equation}
while for all $\alpha<0$ we can establish the redshift property, we ``only'' have the positivity property for $\alpha=0$. In that sense, Prop.~\ref{prop:geb} is sharp.

$\boldsymbol{\m>0}$.
Let us now consider the modified energy current
\begin{equation}
  \label{eq:JMm}
  J^{M;\m}\doteq J^M-\frac{\m}{2}\psi^2\,M^\flat
\end{equation}
where $M^\flat$ is simply the 1-form corresponding to the vectorfield $M$, i.e.~$M^\flat\cdot X=g(M,X)$, and
\begin{equation}
  \label{eq:Mm}
  M=\lr^\alpha\bigl(\bar{Y}+Y\bigr)\,,\qquad(\alpha<0)\,.
\end{equation}
For any solution to the Klein-Gordon equation \eqref{eq:ds:kg} with $\m>0$, this current then has the redshift property, in analogy to \eqref{eq:redshiftM},
\begin{equation}
  \label{eq:redshiftMm}
  \phi\,\nabla\cdot J^{M;\m}\geq \lvert\alpha\rvert \frac{\sqrt{\frac{\Lambda}{3}}}{1+\sqrt{\frac{\Lambda}{3}}r}J^{M;\m}\cdot n\,,
\end{equation}
which then similarly to the above leads to
\begin{equation}
\bigl(1+\sqrt{\frac{\Lambda}{3}}r_2\bigr)^{\lvert\alpha\rvert}\int_{\Sigma_{r_2}}J^{M;\m}\cdot n\,\dm{\gb{r_2}}\leq\bigl(1+\sqrt{\frac{\Lambda}{3}}r_1\bigr)^{\lvert\alpha\rvert}\int_{\Sigma_{r_1}}J^{M;\m}\cdot n\,\dm{\gb{r_1}}\,.
\end{equation}

\begin{prop}\label{prop:gebi}
Let $\psi$ be a solution to the Klein-Gordon equation \eqref{eq:ds:kg} with $\m>0$, then
\begin{multline}
  \label{eq:prop:gebi}
  \int_{\Sigma_{r_2}}\phi\Biggl\{\phi^2\bigl(T\cdot\psi\bigr)^2+\lvert\nablab\psi\rvert^2+\m\psi^2\Biggr\}\dm{\gb{r_2}}\leq\\
  \leq\Bigl(1+\sqrt{\frac{\Lambda}{3}}r_1\Bigr)^{\lvert\alpha\rvert}\:\int_{\Sigma_{r_1}}J^{M;\m}\cdot n\:\dm{\gb{r_1}}
\end{multline}
for any $r_2>r_1>\ch$.
\end{prop}


\subsection{Proofs of the energy estimates in the expanding region}
\label{sec:ds:expanding:c}

In this final section I shall use the double null coordinates \eqref{eq:desitter} to prove the properties of the currents \eqref{eq:JMm} that are essential to the argument made in the previous section. However, these do not rely on the specific coordinate system, and could for example be verified in the spacial coordinates of \eqref{eq:sds:metric:tr} used in our discussion of the Schwarzschild de Sitter case.

$\boldsymbol{\m=0}$.
For a general vectorfield
\begin{equation}
  M=M^u\frac{\partial}{\partial u}+M^v\frac{\partial}{\partial v}
\end{equation}
we calculate
\begin{equation}
\begin{split}
  K^M=&-\frac{\Lambda}{3}\frac{2}{(1+\sqrt{\frac{\Lambda}{3}}r)^2}\frac{\partial M^u}{\partial v}\bigl(\frac{\partial\psi}{\partial u}\bigr)^2
  -\frac{\Lambda}{3}\frac{2}{(1+\sqrt{\frac{\Lambda}{3}}r)^2}\frac{\partial M^v}{\partial u}\bigl(\frac{\partial\psi}{\partial v}\bigr)^2\\
  &-\frac{1}{2}\,\partial_\mu M^\mu\,\lvert\nablab\psi\rvert^2-\frac{1}{2}\frac{2}{1+\sqrt{\frac{\Lambda}{3}}r}\sqrt{\frac{\Lambda}{3}}\,(M\cdot r)\,\lvert\nablab\psi\rvert^2\\
  &+\frac{1}{r}\,(M\cdot r)\,\frac{\Lambda}{3}\Bigl(\frac{2}{1+\sqrt{\frac{\Lambda}{3}}r}\Bigr)^2\frac{\partial\psi}{\partial u}\frac{\partial\psi}{\partial v}\,.
\end{split}
\end{equation}

Here we first set
\begin{equation}
  \label{def:M:hom}
  M\doteq \bar{Y}+Y=\frac{1}{\dd{u}{r}}\pd{u}+\frac{1}{\dd{v}{r}}\pd{v}\,.
\end{equation}
This choice should be viewed as a global redshift vectorfield. Indeed, $\bar{Y}$ and $Y$ separately exploit the redshift effect locally at the cosmological horizons; ($\bar{Y}$ at $u=0$ and $Y$ at $v=0$). While it is clear that $\bar{Y}$ and $Y$ (without a suitable extension) in and by themselves do not give rise to a positive current, the following result shows that the estimate can be \emph{symmetrized}.

\begin{prop}[Positivity Property] \label{prop:geb:b}
Let $M$ be defined by \eqref{def:M:hom}, then
  \begin{equation}
    K^M\geq 0\,.
  \end{equation}
\end{prop}
\begin{proof}
Here
\begin{equation}
  \label{eq:MuMv}
  M^u=\sqrt{\frac{\Lambda}{3}}\frac{(1-uv)^2}{2v}\qquad M^v=\sqrt{\frac{\Lambda}{3}}\frac{(1-uv)^2}{2u}\,.
\end{equation}
Thus
\begin{multline}
  -\frac{\partial M^u}{\partial u}-\frac{\partial M^v}{\partial v}-\frac{2}{1+\sqrt{\frac{\Lambda}{3}}r}\sqrt{\frac{\Lambda}{3}}\,M\cdot r=\\
  =\sqrt{\frac{\Lambda}{3}}(1-uv)+\sqrt{\frac{\Lambda}{3}}(1-uv)-2\sqrt{\frac{\Lambda}{3}}(1-uv)=0\,,
\end{multline}
and
\begin{gather}
  \frac{\partial M^u}{\partial v}=-\sqrt{\frac{\Lambda}{3}}\frac{(1+uv)(1-uv)}{2v^2}\,, \\
  \frac{\partial M^v}{\partial u}=-\sqrt{\frac{\Lambda}{3}}\frac{(1+uv)(1-uv)}{2u^2}\,. 
\end{gather}
Now,
\begin{equation}
  \label{eq:M:pos:symmetrize}
  \frac{2}{r}\,(M\cdot r)\,\frac{\partial\psi}{\partial u}\frac{\partial\psi}{\partial v}\geq
   -\frac{2}{r}\frac{u}{v}\,\Bigl(\frac{\partial\psi}{\partial u}\Bigr)^2  -\frac{2}{r}\frac{v}{u}\,\Bigl(\frac{\partial\psi}{\partial v}\Bigr)^2\,,
\end{equation}
and therefore
\begin{multline}
  K^M\geq \frac{\Lambda}{3}\frac{1}{\lr^2}\Biggl\{\sqrt{\frac{\Lambda}{3}}\biggl[\frac{(1+uv)(1-uv)}{v^2}-4\frac{u}{v}\frac{1-uv}{1+uv}\biggr]\sq{\dd{u}{\psi}}\\
  +\sqrt{\frac{\Lambda}{3}}\biggl[\frac{(1+uv)(1-uv)}{u^2}-4\frac{v}{u}\frac{1-uv}{1+uv}\biggr]\sq{\dd{u}{\psi}}\Biggr\}\displaybreak[0]\\
  =\frac{\Lambda}{3}\frac{1}{\lr^2}\sqrt{\frac{\Lambda}{3}}\frac{(1-uv)^3}{(1+uv)}\Bigl[\frac{1}{v^2}\sq{\dd{u}{\psi}}+\frac{1}{u^2}\sq{\dd{v}{\psi}}\Bigr]\geq 0\,.
\end{multline}
\end{proof}

The energy identity immediately implies:
\begin{cor}\label{prop:geb:c}
For any $r_2>r_1>\ch$ and all solutions~$\psi$ of \eqref{eq:ds:kg} we have
\begin{multline}
  \label{eq:geb:c}
\int_{\Sigma_{r_2}}\phi\,\Bigl\{\phi^2\bigl(T\cdot\psi)^2+\lvert\nablab\psi\rvert^2\Bigr\}\dm{\gb{r_2}}\leq\\
\leq\int_{\Sigma_{r_1}}\phi\,\Bigl\{\phi^2\bigl(T\cdot\psi)^2+\frac{1}{\phi^2}\bigl(\dd{r}{\psi}\bigr)^2+\lvert\nablab\psi\rvert^2\Bigr\}\dm{\gb{r_1}}\,.
\end{multline}
\end{cor}
It is useful to note that the lapse function may be rewritten as
\begin{equation}
  \label{eq:lapse:c}
  \phi=\frac{1}{(uv)^\frac{1}{2}}\frac{1}{1+\sqrt{\frac{\Lambda}{3}}r}\,.
\end{equation}
\begin{proof}
To verify \eqref{eq:geb:c} note that $J^M\cdot n=T(M,\phi V)$, and
\begin{equation}\label{eq:geb:explicit}
  T(M,V)=\frac{1}{2}\frac{\Lambda}{3}\bigl(1-uv\bigr)^2\Bigl[\frac{u}{v}\sq{\dd{u}{\psi}}+\frac{v}{u}\sq{\dd{v}{\psi}}\Bigr]+\sqv{\nablab\psi}\,.
\end{equation}
Moreover,
\begin{equation}
  \bigl(T\cdot\psi\bigr)^2+\bigl(V\cdot\psi\bigr)^2=2\frac{\Lambda}{3}u^2\sq{\dd{u}{\psi}}+2\frac{\Lambda}{3}v^2\sq{\dd{v}{\psi}}\,,
\end{equation}
and $V=\phi^{-2}\partial_r$.
\end{proof}

We have remarked that it is equivalent to consider the vectorfield
\begin{equation}
  \label{eq:M:hom:e}
  M=\frac{1}{1+\sqrt{\frac{\Lambda}{3}} r}\bigl(\bar{Y}+Y\bigr)\,.
\end{equation}
The crucial property \eqref{eq:redshiftM} should here be seen as obtained by prescribing a derivative near the cosmological horizons. Indeed we can think of \eqref{eq:M:hom:e} as obtained by multiplying $\bar{Y}+Y$ by $(-uv)$ and then adding $\bar{Y}+Y$ to ensure that the vectorfield remains timelike.

We shall give a proof of the redshift property \eqref{eq:redshiftM} of the multiplier \eqref{eq:M:hom:e} and its consequences directly in the more general case $\m>0$.

$\boldsymbol{\m>0}$.
Let
\begin{equation}
  J_\mu^{M;\m}[\psi]\doteq J_\mu^M[\psi]-\frac{\m}{2}\,M_\mu\:\psi^2\,,
\end{equation}
where
\begin{equation}
  \label{eq:M:inhom}
  M\doteq\lr^\alpha\bigl(\bar{Y}+Y\bigr)\qquad(\alpha<0)\,.
\end{equation}
Then we have for any solution $\psi$ of \eqref{eq:ds:kg},
\begin{equation}
  \label{eq:JMm:div}
\begin{split}
  \nabla\cdot J^{M;\m}[\psi]&=\bigl(\Box\psi\bigr)\,M\cdot\psi+T_{\mu\nu}[\psi]{}^{(M)}\pi^{\mu\nu}-\frac{\m}{2}\,\nabla_\mu M^\mu\:\psi^2-\m\psi\,M\cdot\psi\\
  &=K^M[\psi]-\frac{\m}{2}\,\nabla\cdot M\:\psi^2\,.
\end{split}
\end{equation}

\begin{prop}\label{pp:redshift:inhom}
Let $\psi$ be a solution to \eqref{eq:ds:kg}, and let $M$ be defined by \eqref{eq:M:inhom}, then
\begin{equation}
  \label{eq:pp:redshift:inhom}
  \phi\,\nabla\cdot J^{M;\m}\geq\lvert\alpha\rvert\frac{\sqrt{\frac{\Lambda}{3}}}{1+\sqrt{\frac{\Lambda}{3}}r}\,J^{M;\m}\cdot n\qquad\big(r>\ch\bigr)\,,
\end{equation}
where $n$ denotes the normal to $\Sigma_r$.
\end{prop}


Note here,
\begin{equation}
  J^{M;\m}\cdot n=J^M\cdot n+\frac{\m}{2}\phi[-g(M,V)]\psi^2\,.
\end{equation}
Since with \eqref{eq:M:inhom}
\begin{equation}
  -g(M,V)=2\lr^\alpha\,,
\end{equation}
we obtain control on the energy density
\begin{multline}
  \label{eq:M:inhom:energy}
  J^{M;\m}\cdot n=\phi\biggl\{2\frac{\Lambda}{3}\frac{1}{\lr^{2-\alpha}}\Bigl[\frac{u}{v}\bigl(\frac{\partial\psi}{\partial u}\bigr)^2+\frac{v}{u}\bigl(\frac{\partial\psi}{\partial v}\bigr)^2\Bigr]\\+\lr^\alpha\lvert\nablab\psi\rvert^2+\m\lr^\alpha\psi^2\biggr\}\,.
\end{multline}

\begin{proof}
Here
\begin{gather}
  M^u=\sqrt{\frac{\Lambda}{3}}\frac{2}{v}\Bigl(\frac{1-uv}{2}\Bigr)^{2-\alpha}\\
  M^v=\sqrt{\frac{\Lambda}{3}}\frac{2}{u}\Bigl(\frac{1-uv}{2}\Bigr)^{2-\alpha}\,.
\end{gather}
Firstly,
\begin{equation}\label{eq:M:inhom:div:angular}
  -\dd{u}{M^u}-\dd{v}{M^v}-\frac{2}{1+\kc r}\kc M\cdot r=(-2\alpha)\kc\lr^{\alpha-1}\,,
\end{equation}
and secondly, by symmetrizing as in \eqref{eq:M:pos:symmetrize},
\begin{multline}
  -\frac{2}{\Omega^2}\dd{v}{M^u}\sq{\dd{u}{\psi}}-\frac{2}{\Omega^2}\dd{u}{M^v}\sq{\dd{v}{\psi}}+\frac{1}{r}\frac{4}{\Omega^2}\dd{u}{\psi}\dd{v}{\psi}\geq\\
  \geq 2\kc^3\Bigl(\frac{1-uv}{2}\Bigr)^{3-\alpha}\Bigl[\frac{(1-uv)^2-\alpha(1+uv)uv}{(1+uv)}\Bigr]\biggl\{\frac{1}{v^2}\sq{\dd{u}{\psi}}+\frac{1}{u^2}\sq{\dd{v}{\psi}}\biggr\}\\
  \geq(-2\alpha)\kc^3\frac{1}{\lr^{3-\alpha}}\Bigl[\frac{u}{v}\sq{\dd{u}{\psi}}+\frac{v}{u}\sq{\dd{v}{\psi}}\Bigr]\,.
\end{multline}
In accordance with \eqref{eq:M:inhom:div:angular} we also find
\begin{equation}
  -\nabla\cdot M=\sqrt{\frac{\Lambda}{3}}\frac{(-2\alpha)}{\lr^{1-\alpha}}\,,
\end{equation}
and thus
\begin{multline}
  \phi\nabla^\mu J_\mu^{M;\m}=\phi\,T_{\mu\nu}[\psi]{}^{(M)}\pi^{\mu\nu}-\frac{\m}{2}\,\phi\,\nabla\cdot M\,\psi^2\displaybreak[0]\\
  =-\alpha\phi\frac{\kc}{1+\kc r}2\frac{\Lambda}{3}\frac{1}{\lr^{2-\alpha}}\biggl[\frac{u}{v}\sq{\dd{u}{\psi}}+\frac{v}{u}\sq{\dd{v}{\psi}}\biggr]\\
  -\alpha\phi\frac{\kc}{1+\kc r}\lr^\alpha\sqv{\nablab\psi}-\alpha\phi\,\m\frac{\kc}{1+\kc r}\lr^\alpha\psi^2\,,
\end{multline}
which yields \eqref{eq:pp:redshift:inhom} by comparison with \eqref{eq:M:inhom:energy}.
\end{proof}

By virtue of the energy identity
\begin{multline}
  \int_{\Sigma_{r_2}}J^{M;\m}\cdot n\,\dm{\gb{r_2}}+\lvert\alpha\rvert\int_{r_1}^{r_2}\ud r \frac{\sqrt{\frac{\Lambda}{3}}}{1+\sqrt{\frac{\Lambda}{3}}r}\int_{\Sigma_r}J^{M;\m}\cdot n\,\dm{\gb{r}}\leq\\
  \leq\int_{\Sigma_{r_1}}J^{M;\m}\cdot n\,\dm{\gb{r_1}}\,,
\end{multline}
and using Lemma~\ref{lemma:gronwall:df}, we can conclude that
\begin{equation}
\label{eq:M:inhom:energy:ub}
\bigl(1+\sqrt{\frac{\Lambda}{3}}r_2\bigr)^{\lvert\alpha\rvert}\int_{\Sigma_{r_2}}J^{M;\m}\cdot n\,\dm{\gb{r_2}}\leq\bigl(1+\sqrt{\frac{\Lambda}{3}}r_1\bigr)^{\lvert\alpha\rvert}\int_{\Sigma_{r_1}}J^{M;\m}\cdot n\,\dm{\gb{r_1}}\,,
\end{equation}
and immediately obtain in view of \eqref{eq:M:inhom:energy} the statement of Prop.~\ref{prop:gebi}.

